Individual Tree Detection in Large-Scale Urban Environments using High-Resolution Multispectral Imagery

We introduce a novel deep learning method for detection of individual trees in urban environments using high-resolution multispectral aerial imagery. We use a convolutional neural network to regress a confidence map indicating the locations of individual trees, which are localized using a peak finding algorithm. Our method provides complete spatial coverage by detecting trees in both public and private spaces, and can scale to very large areas. We performed a thorough evaluation of our method, supported by a new dataset of over 1,500 images and almost 100,000 tree annotations, covering eight cities, six climate zones, and three image capture years. We trained our model on data from Southern California, and achieved a precision of 73.6% and recall of 73.3% using test data from this region. We generally observed similar precision and slightly lower recall when extrapolating to other California climate zones and image capture dates. We used our method to produce a map of trees in the entire urban forest of California, and estimated the total number of urban trees in California to be about 43.5 million. Our study indicates the potential for deep learning methods to support future urban forestry studies at unprecedented scales.

==> Figures/ConfidenceMapComparison/fig_sum_vs_max.tex <==
\begin{figure}
    \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[height=2in]
         {ConfidenceMapComparison/sum_vs_max.pdf}
         \caption{\label{subfig:1dcomparison}}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]
         {ConfidenceMapComparison/val_true_sum.png}
         \caption{\label{subfig:sum}}
         \vspace{0.3in}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\textwidth}
         \vspace{0.2in}
         \includegraphics[width=\textwidth]
         {ConfidenceMapComparison/val_true_max.png}
         \caption{\label{subfig:max}}
         \vspace{0.3in}
    \end{subfigure}
    \caption{\doublespacing Comparison of reduction operations in confidence map construction, in one dimension for visualization purposes.  (a): Construction of a confidence map for two objects located at $x=-0.5$ (blue) and $x=0.5$ (red).  Each object produces a Gaussian centered on its location.  To produce the confidence map, we can apply either a \emph{sum} or \emph{max} reduction operation.  The \emph{sum} reduction (solid black line) produces a single peak in the confidence map at $x=0$, making it difficult to recover the true location of the objects.  In contrast, the \emph{max} reduction (dashed black line) retains the two peaks. 
    (b) and (c): Comparison of confidence maps created with sum reduction and max reduction, respectively.}
    \label{fig:sum_vs_max}
\end{figure}


==> Tables/tab_dataset_comparison.tex <==
\begin{table}
    \centering
    \caption{\doublespacing \added{
    %Comparison of studies with publicly accessible datasets for training and testing tree detection methods.
    Comparison of studies and datasets for training and testing tree detection methods.
        The ``multi-year'' column indicates whether the dataset contains imagery of the same region in different years.  Our study is unique in that it evaluates urban tree detection across geographically distinct cities and climate zones, and includes data for the same areas across multiple years.}}
    \begin{tabular}{lrrlll}
         \textbf{Dataset} & \textbf{Trees}  & \textbf{Sites} & \textbf{Multi-Year} & \textbf{Forest Type} & \textbf{Annotation} \\
         \hline
		 \citet{brandt2020unexpectedly} & 89,899 & 3 & No & Wilderness & Polygon \\
         \citet{ben_weinstein_2022_5914554} & 30,975 & 20 & No & Wilderness & Box \\
         \citet{chen2022transformer} & 98,949 & 1 & No & Wilderness & Point \\
         \hline
         \citet{branson2018google} & 28,678 & 1 & No & Urban & Point \\
         \citet{zamboni2021benchmarking} & 3,382 & 1 & No & Urban & Box  \\
         \citet{das2022geoai} & 6,000 & 1 & No & Urban & Box \\
         \citet{sun2022counting} & 127,969 & 1 & No & Urban & Polygon \\
         \citet{yang2022detecting} & 980 & 1 & No & Urban & Polygon \\
         This study & 95,972 & 8 & Yes & Urban & Point
    \end{tabular}
    \label{tab:dataset_comparison}
\end{table}

==> Tables/tab_method_summary.tex <==
\begin{table}[t]
    \centering
    \caption{\doublespacing Summary of our dataset of annotated \acrshort{naip} tiles in California.  The number of trees listed in the three right-most columns is the number of hand-annotated trees in the study area in each city and in each year. A dash indicates that the area was not annotated for that year.  In total, our dataset contains 95,972 tree annotations.}
    \begin{tabular}{llrrrr}
          &  &  & \multicolumn{3}{c}{\textbf{Year}} \\
         \textbf{City} & \textbf{Climate Zone} & \textbf{Number of Images} &  \textbf{2016} & \textbf{2018} & \textbf{2020}  \\
         \hline
         Bishop  & Interior West & 10 & - & - & 682  \\
         Chico  & Inland Valleys & 99 & - & 8,187 & 8,164  \\
         Claremont & Inland Empire & 92 & 4,858 & 4,880 & 4,678  \\
         Eureka  & Northern California Coast & 21 & - & - & 2,134  \\
         Long Beach & Southern California Coast & 100 & 6,470 & 6,403 & 5,845 \\
         Palm Springs & Southwest Desert  & 100 & 4,433 & 4,707 & 4,109 \\
         Riverside  & Inland Empire & 90 & 5,015 & 4,400 & 4,087 \\
         Santa Monica & Southern California Coast & 92 & 5,824 & 5,830 & 5,841 \\
         \hline
         Total & & 1,651 & 26,600 & 34,407 & 35,565
    \end{tabular}
    \label{tab:dataset_summary}
\end{table}

==> Tables/tab_results.tex <==
\begin{table}[t]
    \centering
    \caption{\doublespacing Results for various configurations of the network tested in our experiments.  Metrics are computed on the test portion of the So.~Cal.~2020 images.  Res.~is the resolution of the output of the network; ``full'' means the output resolution matches the input (0.6 m) whereas ``half'' means the output resolution is half the input resolution.  ``Input'' gives the set of channels in the input raster stack.  ``Att.'' indicates whether or not the attention head was used.  ``Agg.'' indicates the confidence map aggregation method.  $\sigma$ gives the Gaussian kernel width in meters.  The highlighted row represents the configuration with best F-score.  We compare this configuration to others in the text, and qualitatively evaluate its results in Figures \ref{fig:inference}, \ref{fig:crops}, \ref{fig:torrance}, and \ref{fig:heatmap}.}
    \begin{tabular}{llllr|rrrrr}
    \textbf{Res.} & \textbf{Input} & \textbf{Att.} & \textbf{Agg.} & \textbf{$\sigma$ [m]} & \textbf{AP} & \textbf{Precision} & \textbf{Recall} & \textbf{F-Score} & \textbf{RMSE [m]} \\
    \hline
\multicolumn{9}{c}{Varying Density Kernel Width} \\
\hline
Full & RGBNV &   Y & max &  0.900 & \textbf{0.728} &      0.679 &   \textbf{0.757} &   0.716 & 2.120 \\
\rowcolor{lightgray} Full & RGBNV &   Y & max &  1.800 & 0.705 &      0.736 &   0.733 &   \textbf{0.735} & 2.157 \\
Full & RGBNV &   Y & max &  2.700 & 0.670 &      0.761 &   0.688 &   0.723 & 2.249 \\
Full & RGBNV &   Y & max &  3.600 & 0.609 &      \textbf{0.767} &   0.646 &   0.701 & 2.309 \\
\hline
\multicolumn{9}{c}{Varying Input Channels} \\
\hline
Full &    RG &   Y & max &  1.800 & 0.655 &      0.695 &   0.701 &   0.698 & 2.284 \\
Full &   RGN &   Y & max &  1.800 & 0.676 &      0.754 &   0.695 &   0.723 & 2.236 \\
Full &  RGNV &   Y & max &  1.800 & 0.705 &      0.749 &   0.713 &   0.730 & 2.109 \\
Full &   RGB &   Y & max &  1.800 & 0.679 &      0.695 &   0.728 &   0.711 & 2.247 \\
Full &  RGBN &   Y & max &  1.800 & 0.691 &      0.726 &   0.721 &   0.724 & 2.149 \\
\hline
\multicolumn{9}{c}{Sum Reduction instead of Maximum} \\
\hline
Full & RGBNV &   Y & sum &  1.800 & 0.682 &      0.699 &   0.748 &   0.722 & 2.182 \\
\hline
\multicolumn{9}{c}{Half-Resolution Output} \\
\hline
Half & RGBNV &   Y & max &  1.800 & 0.693 &      0.737 &   0.726 &   0.732 & 2.219 \\
\hline
\multicolumn{9}{c}{Without Attention Head} \\
\hline
Full & RGBNV &   N & max &  1.800 & 0.700 &      0.750 &   0.702 &   0.726 & \textbf{2.031} \\
    \end{tabular}
    \label{tab:results}
\end{table}

==> Tables/tab_sigma.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{llrrrr}
    $\sigma$ [px] & $\sigma$ [m] & \textbf{Precision}$\uparrow$ & \textbf{Recall}$\uparrow$ & \textbf{F-Score}$\uparrow$ & \textbf{RMSE} [m]$\downarrow$ \\
    \hline
1.5 & 0.9 & 0.72 & 0.72 & 0.72 & \textbf{3.42} \\
3.0 & 1.8 & \textbf{0.75} & \textbf{0.73} & \textbf{0.74} & 3.51 \\
4.5 & 2.7 & 0.76 & 0.68 & 0.72 & 3.68 \\
6.0 & 3.6 & 0.74 & 0.66 & 0.70 & 3.86 
    \end{tabular}
    \caption{Caption}
    \label{tab:sigma}
\end{table}
